Conservation of Fractional Mean Energy in Dissipative Gases

I show a nontrivial functional giving a conservation quantity in the collisional energy cascade of dissipative Maxwell gases: a fractional-calculus extension of the mean energy. The conservation of this quantity directly leads the power-law energy tail that is stationary during the temporal evolution. In the thermal limit, this quantity naturally reduces to the standard mean energy. This conservation law and its extension to particles with other interactions are demonstrated with a Monte-Carlo simulation for inelastic gases.

==> latexmkrc <==
#!/usr/bin/perl
$latex         = 'pdflatex %O -src-specials -shell-escape -interaction=nonstopmode -synctex=1 main';
$bibtex        = 'pbibtex %O %B';
$dvipdf        = 'dvipdfmx %O -o %D main_supplemental';
$pdf_mode      = 3; # use dvipdfmx

# Use SumatraPDF and atom inverse search
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

# if you do not need to preview in -pvc option (preview document and countinuously update mode)
# $pdf_previewer = 'exit';

